Signal Processing on Product Spaces

We establish a framework for signal processing on product spaces of simplicial and cellular complexes. For simplicity, we focus on the product of two complexes representing time and space, although our results generalize naturally to products of simplicial complexes of arbitrary dimension. Our framework leverages the structure of the eigenmodes of the Hodge Laplacian of the product space to jointly filter along time and space. To this end, we provide a decomposition theorem of the Hodge Laplacian of the product space, which highlights how the product structure induces a decomposition of each eigenmode into a spatial and temporal component. Finally, we apply our method to real world data, specifically for interpolating trajectories of buoys in the ocean from a limited set of observed trajectories.

==> figs/demo.tabular.tex <==
\begin{NiceTabular}{ccc}
    \toprule
    $\nicefrac{\alpha_t}{\alpha_s}$ & \Block{1-2}{$\nicefrac{\|\mathbf{f}^*-\mathbf{f}\|_2}{\|\mathbf{f}\|_2}$} & \\
    & Graph & SC \\
    \midrule
      $0.0$  & $0.518$ & $0.505$ \\
      $0.01$ & $0.065$ & $0.042$ \\
      $0.1$  & $0.101$ & $0.080$ \\
      $1.0$  & $0.110$ & $0.090$ \\
     $10.0$  & $0.108$ & $0.094$ \\
    $\infty$ & $0.716$ & $0.716$ \\
    \bottomrule
\end{NiceTabular}


==> figs/synthetic-experiments-mse.tex <==
\begin{figure}
    \centering
    \small

    \includegraphics[width=\linewidth]{figs/synthetic-experiments-mse.pdf}

    \begin{NiceTabular}{lcccccc}
        \hline
        \Block{2-1}{MSE} & \Block{1-6}{$\nicefrac{\alpha_t}{\alpha_s}$} & & & & & \\
         & $0.0$ & $0.01$ & $0.1$ & $1.0$ & $10.0$ & $\infty$ \\
        \hline
        Mean & $0.0162$ & $0.0032$ & $0.0040$ & $0.0069$ & $0.0442$ & $0.1112$ \\
         Std & $0.0190$ & $0.0027$ & $0.0030$ & $0.0066$ & $0.0290$ & $0.0705$ \\
        \hline
    \end{NiceTabular}

    \caption{
        \textbf{Mean square errors on synthetic experiments with different ratios of temporal and spatial smoothness.}
        The setup follows a matrix-completion style setup with observed and unobserved edge flows.
        The overall and the mean square error only for unobserved edges is given.
    }
    \label{fig:synthetic-experiments-mse}
\end{figure}

